An Empirical Study of Attention Networks for Semantic Segmentation

Semantic segmentation is a vital problem in computer vision. Recently, a common solution to semantic segmentation is the end-to-end convolution neural network, which is much more accurate than traditional methods.Recently, the decoders based on attention achieve state-of-the-art (SOTA) performance on various datasets. But these networks always are compared with the mIoU of previous SOTA networks to prove their superiority and ignore their characteristics without considering the computation complexity and precision in various categories, which is essential for engineering applications. Besides, the methods to analyze the FLOPs and memory are not consistent between different networks, which makes the comparison hard to be utilized. What's more, various methods utilize attention in semantic segmentation, but the conclusion of these methods is lacking. This paper first conducts experiments to analyze their computation complexity and compare their performance. Then it summarizes suitable scenes for these networks and concludes key points that should be concerned when constructing an attention network. Last it points out some future directions of the attention network.

==> figures/plotbatrj.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usepackage{pgfplots}

% \begin{document}

\begin{tikzpicture}
\begin{axis}[
    axis equal=true,
    small,
    width=10cm,
    height=6cm,
    title={Trajectories: \textit{Dataset Room}},
    xlabel={x [m]},
    ylabel={y [m]},
    grid=major,
    grid style={dotted},
    % xmin=0,xmax=85,
    % grid=major,
    legend style={
      at={(0.6,0.75)},
      font=\footnotesize,
    },
]
\addplot [black,thick] table {figures/ba-r4-007.traj-odoerrTruetrj.dat};
\addplot [red,densely dashed] table {figures/ba-r4-007.traj-odoerrOdometrytrj.dat};
\addplot [blue,thin] table {figures/ba-r4-007.traj-odoerrORB-SLAMtrj.dat};
\addplot [green!50!black!80,thick] table {figures/ba-r4-007.traj-odoerrOurstrj.dat};
\legend{Truth,Odometry,ORB-SLAM, Ours},
\end{axis}
\end{tikzpicture}
% \end{document}


==> figures/pose_motivation.tex <==
\begin{tikzpicture}[>=latex,scale=1.0,
  ]

  \def\cameraicon#1#2{
    \begin{scope}[shift={#1}, rotate=#2]
      \draw[thick,fill=white] (-0.3,-0.2) -- (0.3,-0.2) -- (0.3,0.2) -- (0.2,0.2) --
      (0.16,0.24) -- (-0.16,0.24)--(-0.2,0.2)--(-0.3,0.2)--cycle;
      \draw[thick,fill=white] (0,0.02) circle [radius=0.15];
    \end{scope}
  }
  % \draw[gray!50,step=0.5] (0,0) grid (12,6);
  \foreach \x in {0.5,4.5,8.5}
  {
    \draw[thick] (\x,2) rectangle (\x+2.5,3);
    \draw[thick,fill=white] (\x+0.5,2) circle [radius=0.25];
    \draw[thick,fill=white] (\x+2,2) circle [radius=0.25];
    \draw[blue!50] (\x+1.5,5) node {\Large $\bigstar$};
    \draw[blue!50] (\x+0.8,5) node {\small XYZ};
    \cameraicon{(\x+1.25,3)}{0}
    \draw[blue!50,thick,->] (\x+1.25,3) -- (\x+1.5,4.9);
  }
  \foreach \x in {1,2,3,4,5,6,7,8}
  {
    \draw (4.5+\x*0.30,1.75) -- +(-0.25,-0.3);
    \draw[xshift=4cm,yshift=-0.25cm] (4.5+\x*0.30,1.75) -- +(-0.25,-0.3);
  }
  \draw[] (1.75,2.4) node {\small SE(3)};
  \draw[] (5.75,2.4) node {\small SE(2)};
  \draw[] (9.75,2.4) node {\small SE(3)};
  \draw[yshift=0.25cm] (7,1.2) node[fill=white] {\small SE(2)};
  \draw[xshift=4cm] (7,1.2) node[fill=white] {\small SE(2)};
  \draw[thick] (4.5,1.75) -- (7,1.75);
  \draw[thick,xshift=4cm,yshift=-0.25cm] (4.5,1.75) -- (7,1.75);
  \draw[very thick] (9.7,1.5) -- (10,1.65) -- (9.5,1.65) -- (10,1.85) -- (9.5,1.85) --(9.9,2);

  \draw (0.5,0.8) node[below right,align=left] {\small Unconstrained\\ SE(3) poses};
  \draw[xshift=4cm] (0.5,0.8) node[below right,align=left] {\small Deterministic\\ SE(2)-constraints};
  \draw[xshift=8cm] (0.5,0.8) node[below right,align=left] {\small Stochastic\\ SE(2)-constraints\\ on SE(3) poses};

\end{tikzpicture}

